Elasticizing Linux via Joint Disaggregation of Memory and Computation

In this paper, we propose a set of operating system primitives which provides a scaling abstraction to cloud applications in which they can transparently be enabled to support scaled execution across multiple physical nodes as resource needs go beyond that available on a single machine. These primitives include stretch, to extend the address space of an application to a new node, push and pull, to move pages between nodes as needed for execution and optimization, and jump, to transfer execution in a very lightweight manner between nodes. This joint disaggregation of memory and computing allows for transparent elasticity, improving an application's performance by capitalizing on the underlying dynamic infrastructure without needing an application re-write. We have implemented these primitives in a Linux 2.6 kernel, collectively calling the extended operating system, ElasticOS. Our evaluation across a variety of algorithms shows up to 10x improvement in performance over standard network swap.

==> bibliography <==
@misc{CRIU,
  title={CRIU: Checkpoint/Restore In Userspace, July 2011},
  author={EMELYANOV, P}
}
@inproceedings{RamCloud,
	title={Fast crash recovery in RAMCloud},
	author={Ongaro, Diego and Rumble, Stephen M and Stutsman, Ryan and Ousterhout, John and Rosenblum, Mendel},
	booktitle={Proceedings of the Twenty-Third ACM Symposium on Operating Systems Principles},
	pages={29--41},
	year={2011},
	organization={ACM}
}
@inproceedings{Nswap,
	title={Nswap: A network swapping module for linux clusters},
	author={Newhall, Tia and Finney, Sean and Ganchev, Kuzman and Spiegel, Michael},
	booktitle={European Conference on Parallel Processing},
	pages={1160--1169},
	year={2003},
	organization={Springer}
}
@inproceedings{Infiniswap,
	title={Efficient Memory Disaggregation with Infiniswap.},
	author={Gu, Juncheng and Lee, Youngmoon and Zhang, Yiwen and Chowdhury, Mosharaf and Shin, Kang G},
	booktitle={NSDI},
	pages={649--667},
	year={2017}
}
@article{X-Swap,
	title={SwapX: An NVM-based hierarchical swapping framework},
	author={Zhu, Guoliang and Lu, Kai and Wang, Xiaoping and Zhang, Yiming and Zhang, Pengfei and Mittal, Sparsh},
	journal={IEEE Access},
	volume={5},
	pages={16383--16392},
	year={2017},
	publisher={IEEE}
}

@inproceedings{MOSIX,
	title={An organizational grid of federated MOSIX clusters},
	author={Barak, Amnon and Shiloh, Amnon and Amar, Lior},
	booktitle={Cluster Computing and the Grid, 2005. CCGrid 2005. IEEE International Symposium on},
	volume={1},
	pages={350--357},
	year={2005},
	organization={IEEE}
}
@article{milojivcic2000process,
	title={Process migration},
	author={Miloji{\v{c}}i{\'c}, Dejan S and Douglis, Fred and Paindaveine, Yves and Wheeler, Richard and Zhou, Songnian},
	journal={ACM Computing Surveys (CSUR)},
	volume={32},
	number={3},
	pages={241--299},
	year={2000},
	publisher={ACM}
}
@inproceedings{stellner1996cocheck,
	title={CoCheck: Checkpointing and process migration for MPI},
	author={Stellner, Georg},
	booktitle={Parallel Processing Symposium, 1996., Proceedings of IPPS'96, The 10th International},
	pages={526--531},
	year={1996},
	organization={IEEE}
}
@article{smith1988survey,
	title={A survey of process migration mechanisms},
	author={Smith, Jonathan M},
	journal={ACM SIGOPS Operating Systems Review},
	volume={22},
	number={3},
	pages={28--40},
	year={1988},
	publisher={ACM}
} 
@misc{Kerrighed,
	author = {Kerrighed},
	title = {{Kerrighed}},
	howpublished = "\url{http://www.kerrighed.org/wiki/index.php/Main_Page/}", 
	note = "[Online; accessed 6-Feb-2018]"
}
@article{fos,
	title={Factored operating systems (fos): the case for a scalable operating system for multicores},
	author={Wentzlaff, David and Agarwal, Anant},
	journal={ACM SIGOPS Operating Systems Review},
	volume={43},
	number={2},
	pages={76--85},
	year={2009},
	publisher={ACM}
}

@inproceedings{barrelfish,
	title={The multikernel: a new OS architecture for scalable multicore systems},
	author={Baumann, Andrew and Barham, Paul and Dagand, Pierre-Evariste and Harris, Tim and Isaacs, Rebecca and Peter, Simon and Roscoe, Timothy and Sch{\"u}pbach, Adrian and Singhania, Akhilesh},
	booktitle={Proceedings of the ACM SIGOPS 22nd symposium on Operating systems principles},
	pages={29--44},
	year={2009},
	organization={ACM}
}
@inproceedings{hotos13eos,
	title={Towards Elastic Operating Systems.},
	author={Gupta, Amit and Ababneh, Ehab and Han, Richard and Keller, Eric},
	booktitle={HotOS},
	year={2013}
}


@misc{emulab,
	author = {Emulab},
	title = {{emulab}},
	howpublished = "\url{https://www.emulab.net/portal/}", 
	note = "[Online; accessed 6-Feb-2018]"
}
@inproceedings{Farm,
	title={FaRM: Fast remote memory},
	author={Dragojevi{\'c}, Aleksandar and Narayanan, Dushyanth and Hodson, Orion and Castro, Miguel},
	booktitle={Proceedings of the 11th USENIX Conference on Networked Systems Design and Implementation},
	pages={401--414},
	year={2014}
}
@book{munin,
	title={Munin: Distributed shared memory based on type-specific memory coherence},
	author={Bennett, John K and Carter, John B and Zwaenepoel, Willy},
	volume={25},
	number={3},
	year={1990},
	publisher={ACM}
}
@article{KaiLimemory,
	title={Memory coherence in shared virtual memory systems},
	author={Li, Kai and Hudak, Paul},
	journal={ACM Transactions on Computer Systems (TOCS)},
	volume={7},
	number={4},
	pages={321--359},
	year={1989},
	publisher={ACM}
}
@inproceedings{mether,
	title={Mether: Supporting the shared memory model on computing clusters},
	author={Minnich, Ronald G and Pryor, Daniel V},
	booktitle={Compcon Spring'93, Digest of Papers.},
	pages={558--567},
	year={1993},
	organization={IEEE}
}
@inproceedings{BLCR,
	title={Berkeley lab checkpoint/restart (blcr) for linux clusters},
	author={Hargrove, Paul H and Duell, Jason C},
	booktitle={Journal of Physics: Conference Series},
	pages={494},
	year={2006},
	organization={IOP Publishing}
}
@article{mapreduce,
	title={MapReduce: Simplified Data Processing on Large Clusters},
	author={Guo, C and Wu, H and Tan, K and Shiy, L and Zhang, Y and Luz, S},
	journal={Proc. of OSDI 2004, San Francisco, CA, USA},
	year={2004}
}
@inproceedings{fast96,
	title={Fast dynamic process migration},
	author={Roush, Ellard T and Campbell, Roy H},
	booktitle={Distributed Computing Systems, 1996., Proceedings of the 16th International Conference on},
	pages={637--645},
	year={1996},
	organization={IEEE}
}
@inproceedings{apollo,
	author = {Leach, Paul J. and Levine, Paul H. and Hamilton, James A. and Stumpf, Bernard L.},
	title = {The File System of an Integrated Local Network},
	booktitle = {Proceedings of the 1985 ACM Thirteenth Annual Conference on Computer Science},
	series = {CSC '85},
	year = {1985},
	isbn = {0-89791-150-4},
	location = {New Orleans, Louisiana, USA},
	pages = {309--324},
	numpages = {16},
	url = {http://doi.acm.org/10.1145/320599.320696},
	doi = {10.1145/320599.320696},
	acmid = {320696},
	publisher = {ACM},
	address = {New York, NY, USA},
} 
@article{DSM,
	title={Distributed shared memory: A survey of issues and algorithms},
	author={Nitzberg, Bill and Lo, Virginia},
	journal={Computer},
	volume={24},
	number={8},
	pages={52--60},
	year={1991},
	publisher={IEEE}
}

@misc{criu_perf,
		author = {Performance research - CRIU},
   howpublished = {\url{https://criu.org/Performance_research}},
   title = {{Performance research - CRIU}},
   	note = "[Online; accessed 6-Feb-2018]"
   }
   
   
@misc{amazon,
	author = {Amazon},
	howpublished = "\url{ https://aws.amazon.com/ec2/pricing/}", 
	note = "[Online; accessed 6-Feb-2018]"
}
@misc{hadoop,
	author = {Hadoop},
	howpublished = "\url{ http://hadoop.apache.org/}", 
	note = "[Online; accessed 6-Feb-2018]"
}@misc{spark,
author = {Spark},
howpublished = "\url{https://spark.apache.org/}", 
note = "[Online; accessed 6-Feb-2018]"
}
@article{mpi,
	title={Message passing interface (MPI)},
	author={El-Rewini, Hesham and Abd-El-Barr, Mostafa},
	journal={Advanced computer architecture and parallel processing},
	pages={205--233},
	year={2005},
	publisher={Wiley Online Library}
}
@article{de2015partitioned,
	title={Partitioned global address space languages},
	author={De Wael, Mattias and Marr, Stefan and De Fraine, Bruno and Van Cutsem, Tom and De Meuter, Wolfgang},
	journal={ACM Computing Surveys (CSUR)},
	volume={47},
	number={4},
	pages={62},
	year={2015},
	publisher={ACM}
}
@inproceedings{memx,
	title={Memx: Virtualization of cluster-wide memory},
	author={Deshpande, Umesh and Wang, Beilan and Haque, Shafee and Hines, Michael and Gopalan, Kartik},
	booktitle={Parallel Processing (ICPP), 2010 39th International Conference on},
	pages={663--672},
	year={2010},
	organization={IEEE}
}

@ARTICLE{kaili-phd,
	AUTHOR = "{Kai Li}",
	TITLE = "Shared Virtual Memory on Loosely Coupled Microprocessors",
	JOURNAL = "PhD Thesis",
	MONTH = "Spetember",
	YEAR = {1986}	
}

@inproceedings{apollo,
	author = {Leach, Paul J. and Levine, Paul H. and Hamilton, James A. and Stumpf, Bernard L.},
	title = {The File System of an Integrated Local Network},
	booktitle = {Proceedings of the 1985 ACM Thirteenth Annual Conference on Computer Science},
	series = {CSC '85},
	year = {1985},
	isbn = {0-89791-150-4},
	location = {New Orleans, Louisiana, USA},
	pages = {309--324},
	numpages = {16},
	url = {http://doi.acm.org/10.1145/320599.320696},
	doi = {10.1145/320599.320696},
	acmid = {320696},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@book{plka,
	author = {Mauerer, Wolfgang},
	title = {Professional Linux Kernel Architecture},
	year = {2008},
	isbn = {0470343435, 9780470343432},
	publisher = {Wrox Press Ltd.},
	address = {Birmingham, UK, UK},
} 


@article{vdso,
	author = {Beazley, David M. and Ward, Brian D. and Cooke, Ian R.},
	title = {The Inside Story on Shared Libraries and Dynamic Loading},
	journal = {Computing in Science and Engg.},
	issue_date = {September/October 2001},
	volume = {3},
	number = {5},
	month = sep,
	year = {2001},
	issn = {1521-9615},
	pages = {90--97},
	numpages = {8},
	url = {http://dx.doi.org/10.1109/5992.947112},
	doi = {10.1109/5992.947112},
	acmid = {564656},
	publisher = {IEEE Educational Activities Department},
	address = {Piscataway, NJ, USA},
} 


@INPROCEEDINGS{ghost-process, 
	author={G. Vallee and R. Lottiaux and D. Margery and C. Morin}, 
	booktitle={The 4th International Symposium on Parallel and Distributed Computing (ISPDC'05)}, 
	title={Ghost Process: a Sound Basis to Implement Process Duplication, Migration and Checkpoint/Restart in Linux Clusters}, 
	year={2005}, 
	pages={97-104}, 
	keywords={Linux;checkpointing;distributed processing;operating system kernels;workstation clusters;Kerrighed single system image;Linux clusters;distributed system;ghost process;kernel service;operating system;process checkpoint;process duplication;process management;process migration;process restart;process virtualization;Checkpointing;Computer science;Fault tolerance;Government;Kernel;Laboratories;Linux;Mathematics;Operating systems;Resource management;Linux cluster;distributed system;operating system;process virtualization.;single system image}, 
	doi={10.1109/ISPDC.2005.29}, 
	ISSN={2379-5352}, 
	month={July},}

@inproceedings{adaptive-mpi,
	author = {Huang, Chao and Zheng, Gengbin and Kal{\'e}, Laxmikant and Kumar, Sameer},
	title = {Performance Evaluation of Adaptive MPI},
	booktitle = {Proceedings of the Eleventh ACM SIGPLAN Symposium on Principles and Practice of Parallel Programming},
	series = {PPoPP '06},
	year = {2006},
	isbn = {1-59593-189-9},
	location = {New York, New York, USA},
	pages = {12--21},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1122971.1122976},
	doi = {10.1145/1122971.1122976},
	acmid = {1122976},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {MPI, adaptivity, communication optimization, load balancing, processor virtualization},
} 


@article{agora,
	author = {Bisiani, Roberto and Forin, Alessandro},
	title = {Multilanguage Parallel Programming of Heterogeneous Machines},
	journal = {IEEE Trans. Comput.},
	issue_date = {August 1988},
	volume = {37},
	number = {8},
	month = aug,
	year = {1988},
	issn = {0018-9340},
	pages = {930--945},
	numpages = {16},
	url = {http://dx.doi.org/10.1109/12.2245},
	doi = {10.1109/12.2245},
	acmid = {48710},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {Agora, distributed shared memory, event driven invocation, heterogeneous machines, local area network workstations, local area networks, multilanguage parallel applications, parallel programming, performance measurements, programming environments., shared memory abstraction},
} 

@article{mach,
	author = {Rashid, Richard and Tevanian, Avadis and Young, Michael and Golub, David and Baron, Robert and Black, David and Bolosky, William and Chew, Jonathan},
	title = {Machine-independent Virtual Memory Management for Paged Uniprocessor and Multiprocessor Architectures},
	journal = {SIGPLAN Not.},
	issue_date = {Oct. 1987},
	volume = {22},
	number = {10},
	month = oct,
	year = {1987},
	issn = {0362-1340},
	pages = {31--39},
	numpages = {9},
	url = {http://doi.acm.org/10.1145/36205.36181},
	doi = {10.1145/36205.36181},
	acmid = {36181},
	publisher = {ACM},
	address = {New York, NY, USA},
} 


@book{ds-book,
	author = {Coulouris, George and Dollimore, Jean and Kindberg, Tim and Blair, Gordon},
	title = {Distributed Systems: Concepts and Design},
	year = {2011},
	isbn = {0132143011, 9780132143011},
	edition = {5th},
	publisher = {Addison-Wesley Publishing Company},
	address = {USA},
} 

@phdthesis{memnet,
	author = {Delp, Gary Scott},
	title = {The Architecture and Implementation of MEMNET: A High--speed Shared-memory Computer Communication Network},
	year = {1988},
	note = {Order No. GAX88-24208},
	publisher = {University of Delaware},
	address = {Newark, DE, USA},
} 

@book{gorman,
	author = {Gorman, Mel},
	title = {Understanding the Linux Virtual Memory Manager},
	year = {2004},
	isbn = {0131453483},
	publisher = {Prentice Hall PTR},
	address = {Upper Saddle River, NJ, USA},
} 


@misc{upc,
	title = {GASNet},
	howpublished = {\url{http://gasnet.lbl.gov/}},
	note = {Accessed: 2017-06-05}
}

@misc{virtualbox,
	title = {VirtualBox},
	howpublished = {\url{https://www.virtualbox.org}},
	note = {Accessed: 2017-06-05}
}

@misc{kerrig,
	title = {Kerrighed},
	howpublished = {\url{http://www.kerrighed.org/wiki/index.php/Main_Page}},
	note = {Accessed: 2017-06-05}
}

@misc{xtreemos,
	title = {XtreemOS},
	howpublished = {\url{http://www.xtreemos.eu/}},
	note = {Accessed: 2017-06-05}
}




@misc{sparse-page-tables-linux,
	title = {Wikipedia - Page Tables},
	howpublished = {\url{https://en.wikipedia.org/wiki/Page_table}},
	note = {Accessed: 2017-06-05}
}




@misc{emr,
	title = {Amazon's Elastic Map\\Reduce},
	howpublished = {\url{https://aws.amazon.com/emr/}},
	note = {Accessed: 2017-06-05}
}

@misc{nbd,
	title = {Network Block Device},
	howpublished = {\url{https://nbd.sourceforge.io/}},
	note = {Accessed: 2017-06-05}
}


@article{fos,
	author = {Wentzlaff, David and Agarwal, Anant},
	title = {Factored Operating Systems (Fos): The Case for a Scalable Operating System for Multicores},
	journal = {SIGOPS Oper. Syst. Rev.},
	issue_date = {April 2009},
	volume = {43},
	number = {2},
	month = apr,
	year = {2009},
	issn = {0163-5980},
	pages = {76--85},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1531793.1531805},
	doi = {10.1145/1531793.1531805},
	acmid = {1531805},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {factored operating system, multicore operating systems},
} 

@inproceedings{barrelfish,
	author = {Baumann, Andrew and Barham, Paul and Dagand, Pierre-Evariste and Harris, Tim and Isaacs, Rebecca and Peter, Simon and Roscoe, Timothy and Sch\"{u}pbach, Adrian and Singhania, Akhilesh},
	title = {The Multikernel: A New OS Architecture for Scalable Multicore Systems},
	booktitle = {Proceedings of the ACM SIGOPS 22Nd Symposium on Operating Systems Principles},
	series = {SOSP '09},
	year = {2009},
	isbn = {978-1-60558-752-3},
	location = {Big Sky, Montana, USA},
	pages = {29--44},
	numpages = {16},
	url = {http://doi.acm.org/10.1145/1629575.1629579},
	doi = {10.1145/1629575.1629579},
	acmid = {1629579},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {message passing, multicore processors, scalability},
} 

@inproceedings{thrash,
	author = {Denning, Peter J.},
	title = {Thrashing: Its Causes and Prevention},
	booktitle = {Proceedings of the December 9-11, 1968, Fall Joint Computer Conference, Part I},
	series = {AFIPS '68 (Fall, part I)},
	year = {1968},
	location = {San Francisco, California},
	pages = {915--922},
	numpages = {8},
	url = {http://doi.acm.org/10.1145/1476589.1476705},
	doi = {10.1145/1476589.1476705},
	acmid = {1476705},
	publisher = {ACM},
	address = {New York, NY, USA},
} 


@misc{vmotion,
	title = {VMWare's vMotion},
	howpublished = {\url{http://www.vmware.com/products/vsphere/vmotion.html}},
	note = {Accessed: 2017-06-05}
}

@misc{aws-autoscaling,
	title = {AWS auto-scaling.},
	howpublished = {\url{http://aws.amazon.com/autoscaling/}},
	note = {Accessed: 2017-06-05}
}

@misc{azure-autoscaling,
	title = {Microsoft Azure auto-scaling.},
	howpublished = {\url{https://azure.microsoft.com/en-us/features/autoscale/}},
	note = {Accessed: 2017-06-05}
}

@misc{google-autoscaling,
	title = {Google Cloud Platform auto-scaling.},
	howpublished = {\url{https://cloud.google.com/compute/docs/autoscaler/}},
	note = {Accessed: 2017-06-05}
}

@misc{nvme,
	title = {NVM Express},
	howpublished ={\url{http://www.nvmexpress.org/wp-content/uploads/NVM_Express_Revision_1.3.pdf}},
	note = {Accessed: 2017-06-05}
}

@misc{elf,
	title = {Tool Interface Standard (TIS) Executable and Linking Format (ELF) Specification},
	howpublished = {\url{http://refspecs.linuxbase.org/elf/elf.pdf}},
	note = {Accessed: 2017-06-05},
	publisher = {TIS Committee},
	year={1995}
}

@misc{sprite-web,
	title = {The Sprite Operating System},
	howpublished = {\url{https://www2.eecs.berkeley.edu/Research/Projects/CS/sprite/sprite.html}},
	note = {Accessed: 2017-06-05}
}




@techreport{sprite-virt,
	title={Virtual memory for the Sprite operating system},
	author={Nelson, Michael N},
	year={1986},
	institution={CALIFORNIA UNIV BERKELEY COMPUTER SCIENCE DIV}
}


@inproceedings{press,
	added-at = {2011-02-01T00:00:00.000+0100},
	author = {Gong, Zhenhuan and Gu, Xiaohui and Wilkes, John},
	biburl = {http://www.bibsonomy.org/bibtex/2ae83a816f7c58d13cb94a0f05b5a6c96/dblp},
	booktitle = {CNSM},
	crossref = {conf/cnsm/2010},
	ee = {http://dx.doi.org/10.1109/CNSM.2010.5691343},
	interhash = {a0eef68c2449516b52e7a005b9a3482a},
	intrahash = {ae83a816f7c58d13cb94a0f05b5a6c96},
	isbn = {978-1-4244-8908-4},
	keywords = {dblp},
	pages = {9-16},
	publisher = {IEEE},
	timestamp = {2016-01-07T11:44:26.000+0100},
	title = {PRESS: PRedictive Elastic ReSource Scaling for cloud systems.},
	url = {http://dblp.uni-trier.de/db/conf/cnsm/cnsm2010.html#GongGW10},
	year = 2010
}



@INPROCEEDINGS{autoscaling, 
	author={M. Mao and J. Li and M. Humphrey}, 
	booktitle={2010 11th IEEE/ACM International Conference on Grid Computing}, 
	title={Cloud auto-scaling with deadline and budget constraints}, 
	year={2010}, 
	pages={41-48}, 
	keywords={cloud computing;integer programming;virtual machines;Windows Azure platform;attractive computing platform;cloud auto-scaling mechanism;dynamic scalability;performance desire;workload information;Computational modeling;Computer architecture;Delay;Monitoring;Scalability;Time factors;auto-scaling;cloud computing;dynamic scalability;integer programming}, 
	doi={10.1109/GRID.2010.5697966}, 
	ISSN={2152-1085}, 
	month={Oct},}

@misc{gasnet,
	title = {Unified Parallel C},
	howpublished = {\url{https://upc-lang.org/}},
	note = {Accessed: 2017-06-05}
}

@misc{pgas,
	title = {Partitioned Global Address Space},
	howpublished = {\url{http://www.pgas.org/}},
	note = {Accessed: 2017-06-05}
}



@misc{criu,
	title = {Checkpoint/Restore In Userspace (CRIU)},
	howpublished = {\url{https://criu.org/Main_Page}},
	note = {Accessed: 2017-06-05}
}

@inproceedings {farm,
	author = {Aleksandar Dragojevi{\'c} and Dushyanth Narayanan and Miguel Castro and Orion Hodson},
	title = {FaRM: Fast Remote Memory},
	booktitle = {11th USENIX Symposium on Networked Systems Design and Implementation (NSDI 14)},
	year = {2014},
	isbn = {978-1-931971-09-6},
	address = {Seattle, WA},
	pages = {401--414},
	url = {https://www.usenix.org/conference/nsdi14/technical-sessions/dragojevi{\'c}},
	publisher = {USENIX Association},
}

@inproceedings{mosix,
	author = {Barak, A. and Shiloh, A. and Amar, L.},
	title = {An Organizational Grid of Federated MOSIX Clusters},
	booktitle = {Proceedings of the Fifth IEEE International Symposium on Cluster Computing and the Grid - Volume 01},
	series = {CCGRID '05},
	year = {2005},
	isbn = {0-7803-9074-1},
	pages = {350--357},
	numpages = {8},
	url = {http://dl.acm.org/citation.cfm?id=1169222.1169488},
	acmid = {1169488},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
} 

@Inbook{oop,
	author="Dahl, Ole-Johan",
	editor="Owe, Olaf
	and Krogdahl, Stein
	and Lyche, Tom",
	title="The Birth of Object Orientation: the Simula Languages",
	bookTitle="From Object-Orientation to Formal Methods: Essays in Memory of Ole-Johan Dahl",
	year="2004",
	publisher="Springer Berlin Heidelberg",
	address="Berlin, Heidelberg",
	pages="15--25",
	abstract="The development of the programming languages Simula I and Simula 67 is briefly described. An attempt is made also to explain the cultural impact of the languages, in particular the object oriented aspects.",
	isbn="978-3-540-39993-3",
	doi="10.1007/978-3-540-39993-3_3",
	url="http://dx.doi.org/10.1007/978-3-540-39993-3_3"
}



@inproceedings {infiniswap,
	author = {Juncheng Gu and Youngmoon Lee and Yiwen Zhang and Mosharaf Chowdhury and Kang G. Shin},
	title = {Efficient Memory Disaggregation with Infiniswap},
	booktitle = {14th USENIX Symposium on Networked Systems Design and Implementation (NSDI 17)},
	year = {2017},
	isbn = {978-1-931971-37-9},
	address = {Boston, MA},
	pages = {649--667},
	url = {https://www.usenix.org/conference/nsdi17/technical-sessions/presentation/gu},
	publisher = {USENIX Association},
}

@inproceedings {mos,
	author = {A. Barak, A. Shapir, G. Steinberg and A.I. Karshmer},
	title = {A Modular, Distributed UNIX},
	booktitle = {14th USENIX Symposium on Networked Systems Design and Implementation (NSDI 17)},
	year = {1981},
	pages = {740--747},
	month = {January},
}

@INPROCEEDINGS{choices, 
	author={A. Sane and K. MacGregor and R. Campbell}, 
	booktitle={IEEE Workshop on Experimental Distributed Systems}, 
	title={Distributed virtual memory consistency protocols: design and performance}, 
	year={1990}, 
	pages={91-96}, 
	keywords={object-oriented programming;operating systems (computers);protocols;virtual storage;Choices;atomic update;custom-designed protocols;distributed virtual memory consistency protocols;object-oriented framework;page assignment;Application software;Computer science;Control systems;Distributed computing;Memory management;NASA;Operating systems;Parallel processing;Peer to peer computing;Protocols}, 
	doi={10.1109/EDS.1990.138056}, 
	month={Oct},}

@inproceedings{false-sharing,
	author = {Jayasena, Sanath and Amarasinghe, Saman and Abeyweera, Asanka and Amarasinghe, Gayashan and De Silva, Himeshi and Rathnayake, Sunimal and Meng, Xiaoqiao and Liu, Yanbin},
	title = {Detection of False Sharing Using Machine Learning},
	booktitle = {Proceedings of the International Conference on High Performance Computing, Networking, Storage and Analysis},
	series = {SC '13},
	year = {2013},
	isbn = {978-1-4503-2378-9},
	location = {Denver, Colorado},
	pages = {30:1--30:9},
	articleno = {30},
	numpages = {9},
	url = {http://doi.acm.org/10.1145/2503210.2503269},
	doi = {10.1145/2503210.2503269},
	acmid = {2503269},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {false sharing, machine learning, performance events},
} 

@article{pgas1,
	author = {De Wael, Mattias and Marr, Stefan and De Fraine, Bruno and Van Cutsem, Tom and De Meuter, Wolfgang},
	title = {Partitioned Global Address Space Languages},
	journal = {ACM Comput. Surv.},
	issue_date = {July 2015},
	volume = {47},
	number = {4},
	month = may,
	year = {2015},
	issn = {0360-0300},
	pages = {62:1--62:27},
	articleno = {62},
	numpages = {27},
	url = {http://doi.acm.org/10.1145/2716320},
	doi = {10.1145/2716320},
	acmid = {2716320},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {HPC, PGAS, Parallel programming, data access, data distribution, message passing, one-sided communication, survey},
} 


@Inbook{nswap,
	author="Newhall, Tia
	and Finney, Sean
	and Ganchev, Kuzman
	and Spiegel, Michael",
	editor="Kosch, Harald
	and B{\"o}sz{\"o}rm{\'e}nyi, L{\'a}szl{\'o}
	and Hellwagner, Hermann",
	title="Nswap: A Network Swapping Module for Linux Clusters",
	bookTitle="Euro-Par 2003 Parallel Processing: 9th International Euro-Par Conference Klagenfurt, Austria, August 26-29, 2003 Proceedings",
	year="2003",
	publisher="Springer Berlin Heidelberg",
	address="Berlin, Heidelberg",
	pages="1160--1169",
	isbn="978-3-540-45209-6",
	doi="10.1007/978-3-540-45209-6_157",
	url="http://dx.doi.org/10.1007/978-3-540-45209-6_157"
}

@book{guntsch,
	title={Logischer Entwurf eines digitalen Rechenger{\"a}tes mit mehreren asynchron laufenden Trommeln und automatischen Schnellspeicherbetrieb},
	author={G{\"u}ntsch, F.R.T.},
	url={https://books.google.com/books?id=WIokHAAACAAJ},
	year={1957}
}



@INPROCEEDINGS{memx, 
	author={U. Deshpande and B. Wang and S. Haque and M. Hines and K. Gopalan}, 
	booktitle={2010 39th International Conference on Parallel Processing}, 
	title={MemX: Virtualization of Cluster-Wide Memory}, 
	year={2010}, 
	pages={663-672}, 
	keywords={distributed processing;storage management;virtual machines;DRAM;MemX prototype;MemX virtual machine;VM workloads;cluster wide memory virtualization;distributed system;host machine;large memory workloads;Bridges;Driver circuits;Memory management;Protocols;Random access memory;Servers;Virtual machine monitors;Cluster;Gigabit Ethernet;Hypervisor;Memory;Virtualization}, 
	doi={10.1109/ICPP.2010.74}, 
	ISSN={0190-3918}, 
	month={Sept},}

@ARTICLE{auto-parallel,
	author={Banerjee, U. and Eigenmann, R. and Nicolau, A and Padua, D.A},
	journal={Proceedings of the IEEE},
	title={Automatic program parallelization},
	year={1993},
	month={Feb},
	volume={81},
	number={2},
	pages={211-243},
	keywords={automatic programming;parallel programming;program compilers;automatic program parallelization techniques;dependence analysis techniques;do-loop transformations;parallelizing compilers;program transformations;recursive routines;straight-line code parallelization;Character generation;Computer languages;Computer science;Frequency;Parallel processing;Parallel programming;Power generation;Problem-solving;Research and development;US Department of Energy},
	doi={10.1109/5.214548},
	ISSN={0018-9219},}

@inproceedings{pgo,
	author = {Homescu, Andrei and Neisius, Steven and Larsen, Per and Brunthaler, Stefan and Franz, Michael},
	title = {Profile-guided Automated Software Diversity},
	booktitle = {Proceedings of the 2013 IEEE/ACM International Symposium on Code Generation and Optimization (CGO)},
	series = {CGO '13},
	year = {2013},
	isbn = {978-1-4673-5524-7},
	pages = {1--11},
	numpages = {11},
	url = {http://dx.doi.org/10.1109/CGO.2013.6494997},
	doi = {10.1109/CGO.2013.6494997},
	acmid = {2495928},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {NOP insertion,Profiling, Automated Software Diversity, Compilers, Cold,Code},
} 



@techreport{gasnet,
	author    = "{Dan Bonachea}",
	title     = "{GASNet Specification, v1.1}",
	institution = "University of California at Berkeley",
	address  = "Berkeley, CA, USA",
	year      = "2002",
}



@article{fos,
	author = {Wentzlaff, David and Agarwal, Anant},
	title = {Factored Operating Systems (Fos): The Case for a Scalable Operating System for Multicores},
	journal = {SIGOPS Oper. Syst. Rev.},
	issue_date = {April 2009},
	volume = {43},
	number = {2},
	month = apr,
	year = {2009},
	issn = {0163-5980},
	pages = {76--85},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/1531793.1531805},
	doi = {10.1145/1531793.1531805},
	acmid = {1531805},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {factored operating system, multicore operating systems},
} 

@inproceedings{sel4,
	author = {Klein, Gerwin and Elphinstone, Kevin and Heiser, Gernot and Andronick, June and Cock, David and Derrin, Philip and Elkaduwe, Dhammika and Engelhardt, Kai and Kolanski, Rafal and Norrish, Michael and Sewell, Thomas and Tuch, Harvey and Winwood, Simon},
	title = {seL4: Formal Verification of an OS Kernel},
	booktitle = {Proceedings of the ACM SIGOPS 22Nd Symposium on Operating Systems Principles},
	series = {SOSP '09},
	year = {2009},
	isbn = {978-1-60558-752-3},
	location = {Big Sky, Montana, USA},
	pages = {207--220},
	numpages = {14},
	url = {http://doi.acm.org/10.1145/1629575.1629596},
	doi = {10.1145/1629575.1629596},
	acmid = {1629596},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {isabelle/hol, l4, microkernel, sel4},
} 

@inproceedings{mapreduce,
	author = {Dean, Jeffrey and Ghemawat, Sanjay},
	title = {MapReduce: Simplified Data Processing on Large Clusters},
	booktitle = {Proceedings of the 6th Conference on Symposium on Opearting Systems Design \& Implementation - Volume 6},
	series = {OSDI'04},
	year = {2004},
	location = {San Francisco, CA},
	pages = {10--10},
	numpages = {1},
	url = {http://dl.acm.org/citation.cfm?id=1251254.1251264},
	acmid = {1251264},
	publisher = {USENIX Association},
	address = {Berkeley, CA, USA},
} 
@article{locks-cache-coherence,
	author = {Mellor-Crummey, John M. and Scott, Michael L.},
	title = {Algorithms for Scalable Synchronization on Shared-memory Multiprocessors},
	journal = {ACM Trans. Comput. Syst.},
	issue_date = {Feb. 1991},
	volume = {9},
	number = {1},
	month = feb,
	year = {1991},
	issn = {0734-2071},
	pages = {21--65},
	numpages = {45},
	url = {http://doi.acm.org/10.1145/103727.103729},
	doi = {10.1145/103727.103729},
	acmid = {103729},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@INPROCEEDINGS{mether, 
	author={R. G. Minnich and D. V. Pryor}, 
	booktitle={Digest of Papers. Compcon Spring}, 
	title={Mether: supporting the shared memory model on computing clusters}, 
	year={1993}, 
	pages={558-567}, 
	keywords={computer networks;shared memory systems;storage management;C90 supercomputer;MNFS;Mether address space;Mether-NFS;Monte Carlo radiative heat transfer simulation;SPARCStations;SunOS;computing clusters;consistency semantics;distributed shared memory;file system space;modified NFS system;operating system;parallel application;shared memory model;shared memory space;synchronization;Application software;Assembly;Computer networks;Distributed computing;File systems;Operating systems;Sun;Supercomputers;Time sharing computer systems;Trademarks}, 
	doi={10.1109/CMPCON.1993.289734}, 
	month={Feb},}

@article{clouds,
	title={An implementation of distributed shared memory},
	author={Ramachandran, Umakishore and Khalidi, M Yousef A},
	journal={Software: Practice and Experience},
	volume={21},
	number={5},
	pages={443--464},
	year={1991},
	publisher={Wiley Online Library}
}

@inproceedings{false-sharing,
	author = {Bolosky, William J. and Scott, Michael L.},
	title = {False Sharing and Its Effect on Shared Memory Performance},
	booktitle = {USENIX Systems on USENIX Experiences with Distributed and Multiprocessor Systems - Volume 4},
	series = {Sedms'93},
	year = {1993},
	location = {San Diego, California},
	pages = {3--3},
	numpages = {1},
	url = {http://dl.acm.org/citation.cfm?id=1295480.1295483},
	acmid = {1295483},
	publisher = {USENIX Association},
	address = {Berkeley, CA, USA},
} 


@inproceedings{mpi-elasiticty,
	author = {Rajan, Dinesh and Canino, Anthony and Izaguirre, Jesus A. and Thain, Douglas},
	title = {Converting a High Performance Application to an Elastic Cloud Application},
	booktitle = {Proceedings of the 2011 IEEE Third International Conference on Cloud Computing Technology and Science},
	series = {CLOUDCOM '11},
	year = {2011},
	isbn = {978-0-7695-4622-3},
	pages = {383--390},
	numpages = {8},
	url = {https://doi.org/10.1109/CloudCom.2011.58},
	doi = {10.1109/CloudCom.2011.58},
	acmid = {2116233},
	publisher = {IEEE Computer Society},
	address = {Washington, DC, USA},
	keywords = {Elastic applications, cloud computing, distributed computing, high performance applications, replica exchange, molecular dynamics},
} 


@inproceedings{fos-cloud,
	author = {Wentzlaff, David and Gruenwald,III, Charles and Beckmann, Nathan and Modzelewski, Kevin and Belay, Adam and Youseff, Lamia and Miller, Jason and Agarwal, Anant},
	title = {An Operating System for Multicore and Clouds: Mechanisms and Implementation},
	booktitle = {Proceedings of the 1st ACM Symposium on Cloud Computing},
	series = {SoCC '10},
	year = {2010},
	isbn = {978-1-4503-0036-0},
	location = {Indianapolis, Indiana, USA},
	pages = {3--14},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/1807128.1807132},
	doi = {10.1145/1807128.1807132},
	acmid = {1807132},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {cloud computing, multicores, scalable operating systems, single system image},
} 

@inproceedings{barrelfish,
	author = {Baumann, Andrew and Barham, Paul and Dagand, Pierre-Evariste and Harris, Tim and Isaacs, Rebecca and Peter, Simon and Roscoe, Timothy and Sch\"{u}pbach, Adrian and Singhania, Akhilesh},
	title = {The Multikernel: A New OS Architecture for Scalable Multicore Systems},
	booktitle = {Proceedings of the ACM SIGOPS 22Nd Symposium on Operating Systems Principles},
	series = {SOSP '09},
	year = {2009},
	isbn = {978-1-60558-752-3},
	location = {Big Sky, Montana, USA},
	pages = {29--44},
	numpages = {16},
	url = {http://doi.acm.org/10.1145/1629575.1629579},
	doi = {10.1145/1629575.1629579},
	acmid = {1629579},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {message passing, multicore processors, scalability},
} 

@inproceedings{eos,
	author = {Gupta, Amit and Ababneh, Ehab and Han, Richard and Keller, Eric},
	title = {Towards Elastic Operating Systems},
	booktitle = {Proceedings of the 14th USENIX Conference on Hot Topics in Operating Systems},
	series = {HotOS'13},
	year = {2013},
	location = {Santa Ana Pueblo, New Mexcio},
	pages = {16--16},
	numpages = {1},
	url = {http://dl.acm.org/citation.cfm?id=2490483.2490499},
	acmid = {2490499},
	publisher = {USENIX Association},
	address = {Berkeley, CA, USA},
} 


@techreport{ams,
	Author = {Mainwaring, Alan M. and Culler, David E.},
	Title = {Active Message Applications Programming Interface and Communication Subsystem Organization},
	Institution = {EECS Department, University of California, Berkeley},
	Year = {1996},
	Month = {Oct},
	URL = {http://www.eecs.berkeley.edu/Pubs/TechRpts/1996/5768.html},
	Number = {UCB/CSD-96-918},
}

@techreport{upc,
	author    = "{UPC Consortium}",
	title     = "{UPC Language and Library Specifications, v1.3}",
	institution = "Lawrence Berkeley National Lab",
	address  = "Berkeley, CA, USA",
	year = "2013",
	month = "November",
}

@INPROCEEDINGS{munin,
	AUTHOR = "{J.K. Bennett, J.B. Carter, and W. Zwaenepoel}",
	TITLE = "Munin: Distributed shared memory based on type--specific memory coherence",
	BOOKTITLE = "ACM SIGPLAN Symposium on Principles and Practice of Parallel Programming (PPoPP)",
	PAGES = "168-176",
	MONTH = "March", 
	YEAR = {1990}	
}


@inproceedings{distributed-ht,
	author = {Gupta, Anjali and Liskov, Barbara and Rodrigues, Rodrigo},
	title = {Efficient Routing for Peer-to-peer Overlays},
	booktitle = {Proceedings of the 1st Conference on Symposium on Networked Systems Design and Implementation - Volume 1},
	series = {NSDI'04},
	year = {2004},
	location = {San Francisco, California},
	pages = {9--9},
	numpages = {1},
	url = {http://dl.acm.org/citation.cfm?id=1251175.1251184},
	acmid = {1251184},
	publisher = {USENIX Association},
	address = {Berkeley, CA, USA},
} 


@inproceedings{consistent-hashing,
	author = {Karger, David and Lehman, Eric and Leighton, Tom and Panigrahy, Rina and Levine, Matthew and Lewin, Daniel},
	title = {Consistent Hashing and Random Trees: Distributed Caching Protocols for Relieving Hot Spots on the World Wide Web},
	booktitle = {Proceedings of the Twenty-ninth Annual ACM Symposium on Theory of Computing},
	series = {STOC '97},
	year = {1997},
	isbn = {0-89791-888-6},
	location = {El Paso, Texas, USA},
	pages = {654--663},
	numpages = {10},
	url = {http://doi.acm.org/10.1145/258533.258660},
	doi = {10.1145/258533.258660},
	acmid = {258660},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@inproceedings{chord,
	author = {Stoica, Ion and Morris, Robert and Karger, David and Kaashoek, M. Frans and Balakrishnan, Hari},
	title = {Chord: A Scalable Peer-to-peer Lookup Service for Internet Applications},
	booktitle = {Proceedings of the 2001 Conference on Applications, Technologies, Architectures, and Protocols for Computer Communications},
	series = {SIGCOMM '01},
	year = {2001},
	isbn = {1-58113-411-8},
	location = {San Diego, California, USA},
	pages = {149--160},
	numpages = {12},
	url = {http://doi.acm.org/10.1145/383059.383071},
	doi = {10.1145/383059.383071},
	acmid = {383071},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@ARTICLE{compare,
	author = {Fred Douglis and M. Frans Kaashoek and John K. Ousterhout and Andrew S. Tanenbaum},
	title = {A Comparison of Two Distributed Systems: Amoeba and Sprite},
	journal = {ACM Transactions on Computer Systems},
	year = {1991},
	volume = {4},
	pages = {Fall}
}

@INPROCEEDINGS{sprite-migrate,
	author = {Fred Douglis},
	title = {Experience with Process Migration in Sprite},
	booktitle = {Proceedings of USENIX Workshop on Distributed an Multiprocessor Systems},
	year = {1989},
	pages = {59--72}
}

@article{kerrighed,
	author = {Morin, Christine and Gallard, Pascal and Lottiaux, Renaud and Vall{\'e}e, Geoffroy},
	title = {Towards an Efficient Single System Image Cluster Operating System},
	journal = {Future Gener. Comput. Syst.},
	issue_date = {May 2004},
	volume = {20},
	number = {4},
	month = may,
	year = {2004},
	issn = {0167-739X},
	pages = {505--521},
	numpages = {17},
	url = {http://dx.doi.org/10.1016/S0167-739X(03)00170-5},
	doi = {10.1016/S0167-739X(03)00170-5},
	acmid = {1006385},
	publisher = {Elsevier Science Publishers B. V.},
	address = {Amsterdam, The Netherlands, The Netherlands},
	keywords = {cluster, distributed system, operating system, single system image},
} 



@inproceedings{ramcloud,
	author = {Ongaro, Diego and Rumble, Stephen M. and Stutsman, Ryan and Ousterhout, John and Rosenblum, Mendel},
	title = {Fast Crash Recovery in RAMCloud},
	booktitle = {Proceedings of the Twenty-Third ACM Symposium on Operating Systems Principles},
	series = {SOSP '11},
	year = {2011},
	isbn = {978-1-4503-0977-6},
	location = {Cascais, Portugal},
	pages = {29--41},
	numpages = {13},
	url = {http://doi.acm.org/10.1145/2043556.2043560},
	doi = {10.1145/2043556.2043560},
	acmid = {2043560},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {crash recovery, main memory databases, scalability, storage systems},
} 

@article{numa,
	author = {Lameter, Christoph},
	title = {An Overview of Non-uniform Memory Access},
	journal = {Commun. ACM},
	issue_date = {September 2013},
	volume = {56},
	number = {9},
	month = sep,
	year = {2013},
	issn = {0001-0782},
	pages = {59--54},
	numpages = {-4},
	url = {http://doi.acm.org/10.1145/2500468.2500477},
	doi = {10.1145/2500468.2500477},
	acmid = {2500477},
	publisher = {ACM},
	address = {New York, NY, USA},
} 

@techreport{tui,
	author = {Smith, Peter and Hutchinson, Norman C.},
	title = {Heterogeneous Process Migration: The Tui System},
	year = {1996},
	source = {http://www.ncstrl.org:8900/ncstrl/servlet/search?formname=detail\&id=oai%3Ancstrlh%3Aubc_cs%3Ancstrl.ubc_cs%2F%2FTR-96-04},
	publisher = {University of British Columbia},
	address = {Vancouver, BC, Canada, Canada},
} 

@article{ivy,
	author = {Li, Kai and Hudak, Paul},
	title = {Memory Coherence in Shared Virtual Memory Systems},
	journal = {ACM Trans. Comput. Syst.},
	issue_date = {Nov. 1989},
	volume = {7},
	number = {4},
	month = nov,
	year = {1989},
	issn = {0734-2071},
	pages = {321--359},
	numpages = {39},
	url = {http://doi.acm.org/10.1145/75104.75105},
	doi = {10.1145/75104.75105},
	acmid = {75105},
	publisher = {ACM},
	address = {New York, NY, USA},
} 


@misc{scalemp,
	key="ScaleMP",
	title = {vSMP Foundation},
	howpublished = "\url{http://www.scalemp.com/products/vsmp-foundation/}",
	year = {2014}, 
	note = "[Online; accessed 01-July-2014]"
}

@misc{mpi,
	key="mpi",
	title = {MPI Standard},
	howpublished = "\url{http://www-unix.mcs.anl.gov/mpi/mpi-standard/mpi-report-1.0.ps}",
	year = {1995}, 
	note = "[Online; accessed 01-July-2014]"
}

@misc{linux,
	key="Linux",
	title = {Linux},
	howpublished = "\url{http://www.linux.org}",
	note = "[Online; accessed 01-July-2014]"
}

@misc{myrinet,
	title = {Myrinet},
	author = "Myricom",
	howpublished = "\url{http://www.myricom.com/scs/myrinet/overview/}",
	ORGANIZATION = "Myricom",
	note = "[Online; accessed 01-July-2014]"
}


@misc{intel,
	title = {Intel's 48-core processor},
	author = "Intel",
	howpublished = "\url{http://www.intel.com/pressroom/archive/releases/2009/20091202comp_sm.htm}",
	ORGANIZATION = "Intel",
	note = "[Online; accessed 01-July-2014]"
}

@misc{infiniband,
	key="infiniband",
	title = "{InfiniBand Trade Association}",
	howpublished = "\url{http://www.infinibandta.org/}",
	note = "[Online; accessed 01-July-2014]"
}

@INPROCEEDINGS{disom,
	AUTHOR = "{Paulo Guedes, Miguel Castro, and Nuno Neves}",
	TITLE = "The DiSOM distributed shared object memory",
	BOOKTITLE = "6th workshop on ACM SIGOPS European workshop: Matching operating systems to application needs",
	PAGES = "138-140",
	YEAR = {1994}	
}

@INPROCEEDINGS{tread,
	AUTHOR = "{Pete Keleher , Alan L. Cox , Sandhya Dwarkadas , Willy Zwaenepoel}",
	TITLE = " TreadMarks: Distributed Shared Memory on Standard Workstations and Operating Systems",
	BOOKTITLE = "WINTER USENIX CONFERENCE",
	YEAR = {1994}	
}

@inproceedings{vm-migration,
	author = {Clark, Christopher and Fraser, Keir and Hand, Steven and Hansen, Jacob Gorm and Jul, Eric and Limpach, Christian and Pratt, Ian and Warfield, Andrew},
	title = {Live Migration of Virtual Machines},
	booktitle = {Proceedings of the 2Nd Conference on Symposium on Networked Systems Design \& Implementation - Volume 2},
	series = {NSDI'05},
	year = {2005},
	pages = {273--286},
	numpages = {14},
	url = {http://dl.acm.org/citation.cfm?id=1251203.1251223},
	acmid = {1251223},
	publisher = {USENIX Association},
	address = {Berkeley, CA, USA},
} 


@techreport{TSX,
	added-at = {2013-09-06T17:22:08.000+0200},
	author = {Intel},
	biburl = {https://www.bibsonomy.org/bibtex/2a15a0cafb4a75d8d74628b3a72ceade3/davef},
	institution = {Intel},
	interhash = {cacfe366b5b193f85533c3fb6bf8366b},
	intrahash = {a15a0cafb4a75d8d74628b3a72ceade3},
	keywords = {diss hardware specification standard},
	month = {August},
	number = {319433-014},
	timestamp = {2013-11-13T22:34:29.000+0100},
	title = {Intel Architecture Instruction Set Extensions Programming Reference},
	url = {http://download-software.intel.com/sites/default/files/319433-014.pdf},
	year = 2012
}

@inproceedings{elastic-mpi-2016,
	author = {Compr{\'e}s, Isa\'{\i}as and Mo-Hellenbrand, Ao and Gerndt, Michael and Bungartz, Hans-Joachim},
	title = {Infrastructure and API Extensions for Elastic Execution of MPI Applications},
	booktitle = {Proceedings of the 23rd European MPI Users' Group Meeting},
	series = {EuroMPI 2016},
	year = {2016},
	isbn = {978-1-4503-4234-6},
	location = {Edinburgh, United Kingdom},
	pages = {82--97},
	numpages = {16},
	url = {http://doi.acm.org/10.1145/2966884.2966917},
	doi = {10.1145/2966884.2966917},
	acmid = {2966917},
	publisher = {ACM},
	address = {New York, NY, USA},
	keywords = {Elastic Computing, MPI, MPICH, Malleable Applications, Message Passing, Resource Aware Computing, SLURM},
} 

@INPROCEEDINGS{elastic-mpi-2011, 
	author={A. Raveendran and T. Bicer and G. Agrawal}, 
	booktitle={2011 IEEE International Symposium on Parallel and Distributed Processing Workshops and Phd Forum}, 
	title={A Framework for Elastic Execution of Existing MPI Programs}, 
	year={2011}, 
	pages={940-947}, 
	keywords={cloud computing;message passing;HPC applications;MPI programs;cloud resources;cost constraint;resource allocation;time constraint;Arrays;Cloud computing;Elasticity;Monitoring;Resource management;Runtime}, 
	doi={10.1109/IPDPS.2011.240}, 
	ISSN={1530-2075}, 
	month={May},}

@inproceedings{treadmarks,
	author = {Keleher, Pete and Cox, Alan L. and Dwarkadas, Sandhya and Zwaenepoel, Willy},
	title = {TreadMarks: Distributed Shared Memory on Standard Workstations and Operating Systems},
	booktitle = {Proceedings of the USENIX Winter 1994 Technical Conference on USENIX Winter 1994 Technical Conference},
	series = {WTEC'94},
	year = {1994},
	location = {San Francisco, California},
	pages = {10--10},
	numpages = {1},
	url = {http://dl.acm.org/citation.cfm?id=1267074.1267084},
	acmid = {1267084},
	publisher = {USENIX Association},
	address = {Berkeley, CA, USA},
} 


@article{mapreduce,
	author = {Dean, Jeffrey and Ghemawat, Sanjay},
	title = {MapReduce: Simplified Data Processing on Large Clusters},
	journal = {Commun. ACM},
	issue_date = {January 2008},
	volume = {51},
	number = {1},
	month = jan,
	year = {2008},
	issn = {0001-0782},
	pages = {107--113},
	numpages = {7},
	url = {http://doi.acm.org/10.1145/1327452.1327492},
	doi = {10.1145/1327452.1327492},
	acmid = {1327492},
	publisher = {ACM},
	address = {New York, NY, USA},
}

@ARTICLE{amoeba,
	author = {Andrew S. Tanenbaum and M. Frans Kaashoek and Robbert Van Renesse and Henri E. Bal},
	title = {The Amoeba Distributed Operating System - A Status Report},
	journal = {Computer Communications},
	year = {1991},
	volume = {14},
	pages = {324--335}
}


